Efficient Encoders for Streaming Sequence Tagging

A naive application of state-of-the-art bidirectional encoders for streaming sequence tagging would require encoding each token from scratch for each new token in an incremental streaming input (like transcribed speech). The lack of re-usability of previous computation leads to a higher number of Floating Point Operations (or FLOPs) and higher number of unnecessary label flips. Increased FLOPs consequently lead to higher wall-clock time and increased label flipping leads to poorer streaming performance. In this work, we present a Hybrid Encoder with Adaptive Restart (HEAR) that addresses these issues while maintaining the performance of bidirectional encoders over the offline (or complete) inputs while improving performance on streaming (or incomplete) inputs. HEAR has a Hybrid unidirectional-bidirectional encoder architecture to perform sequence tagging, along with an Adaptive Restart Module (ARM) to selectively guide the restart of bidirectional portion of the encoder. Across four sequence tagging tasks, HEAR offers FLOP savings in streaming settings upto 71.1% and also outperforms bidirectional encoders for streaming predictions by upto +10% streaming exact match.

==> radar.tex <==
\begin{tikzpicture}[scale=0.3]
\tkzKiviatDiagramFromFile[
        scale=.5,
        label distance=1cm,
        gap     = 1.75,label space=3,  
        lattice = 12]{tableae.dat}

\tkzKiviatLineFromFile[thick,
                       color      = red,
                       mark       = ball,
                       ball color = red,
                       mark size  = 4pt,
                       fill       = red!20]{tableae.dat}{1} 
\tkzKiviatLineFromFile[thick,
                       color      = blue,
                       mark       = ball,
                       ball color = blue,
                       mark size  = 4pt,
                       fill       = blue!20]{tableae.dat}{2}
\tkzKiviatLineFromFile[thick,
                       color      = green,
                       mark       = ball,
                       ball color = green,
                       mark size  = 4pt,
                       fill       = green!20]{tableae.dat}{3}
\tkzKiviatLineFromFile[thick,
                       color      = brown,
                       mark       = ball,
                       ball color = brown,
                       mark size  = 4pt,
                       fill       = brown!20]{tableae.dat}{4}
% \tkzKiviatLineFromFile[thick,
%                        color      = cyan,
%                        mark       = ball,
%                        ball color = cyan,
%                        mark size  = 4pt,
%                        fill       = cyan!20]{tableae.dat}{5}
\end{tikzpicture}
\begin{tikzpicture}
    \draw[draw=black] (-0.1,-0.2) rectangle ++(8,1);
    \draw [thick, red] (0,0.5) -- (0.5,0.5); 
    \node at (1.5,0.5) {BiDi};
    \draw [thick, blue] (2.75,0.5) -- (3.25,0.5); 
    \node at (4.25,0.5) {pBiDi};
    \draw [thick, green] (0,0) -- (0.5,0); 
    \node at (1.5,0) {Bidi + ARM};
    \draw [thick, brown] (2.75,0) -- (3.25,0); 
    \node at (4.25,0) {PEAR};
    % \draw [thick, yellow] (5.50,0) -- (6,0); 
    % \node at (7,0) {Bidi + ARM};
\end{tikzpicture}
% \begin{tikzpicture}
% \tkzKiviatDiagram[scale=1.25,label distance=.5cm,
%         radial  = 5,
%         gap     = 1,  
%         lattice = 5]{McCabe,LOC,Live Variables,Halstead N,Variablenspanne}
% \tkzKiviatLine[thick,color=blue,mark=none,
%                fill=blue!20,opacity=.5](3,3.5,3,3.5,3)
% \tkzKiviatLine[thick,color=darkgray,
%                fill=green!20,opacity=.5](0.5,1,0.5,0.75,1) 
% \tkzKiviatLine[ultra thick,mark=ball,
%                  mark size=4pt,color =Maroon](2,3.75,1,1.5,2)    
% \tkzKiviatGrad[prefix=,unity=100,suffix=\ \texteuro](1)  
% \end{tikzpicture}

==> tables.tex <==
\begin{table*}[h!]
\small
\centering\begin{tabular}{c c c c c}
\toprule
Model & snips & chunk & ner & srl \\
\midrule
UniDi & 82.89 & 75.76 & 72.09 & 27.84 \\
\encoder~ (uni=1) & 74.96 & 77.55 & 78.81 & 54.26 \\
\encoder~ (uni=2) & 72.55 & 77.72 & 79.28 & 51.75 \\
\encoder~ (uni=3) & 74.84 & 77.67 & 79.51 & 49.06 \\
BiDi & 75.08 & 78.07 & 78.67 & 43.6 \\
\bottomrule
\end{tabular}
\caption{Streaming EM without adapter}
\end{table*}

\begin{table*}[h!]
\small
\centering\begin{tabular}{c c c c c}
\toprule
Model & snips & chunk & ner & srl \\
\midrule
UniDi & 100.0 & 100.0 & 100.0 & 100.0 \\
\encoder~ (uni=1) & 79.07 & 92.82 & 88.23 & 67.89 \\
\encoder~ (uni=2) & 76.31 & 91.87 & 88.15 & 64.62 \\
\encoder~ (uni=3) & 78.2 & 91.55 & 88.25 & 61.46 \\
BiDi & 78.21 & 91.62 & 87.21 & 55.96 \\
\bottomrule
\end{tabular}
\caption{RC without adapter}
\end{table*}

\begin{table*}[h!]
\small
\centering\begin{tabular}{c c c c c}
\toprule
Model & snips & chunk & ner & srl \\
\midrule
UniDi & 0.0 & 0.0 & 0.0 & 0.0 \\
\encoder~ (uni=1) & 14.64 & 4.54 & 8.33 & 23.86 \\
\encoder~ (uni=2) & 16.71 & 4.84 & 8.27 & 27.9 \\
\encoder~ (uni=3) & 15.68 & 4.82 & 8.11 & 29.93 \\
BiDi & 15.86 & 4.72 & 8.73 & 33.02 \\
\bottomrule
\end{tabular}
\caption{EO without adapter}
\end{table*}

\begin{table*}[h!]
\small
\centering\begin{tabular}{c c c c c}
\toprule
Model & snips & chunk & ner & srl \\
\midrule
UniDi & 86.76 & 88.13 & 73.76 & 56.36 \\
\encoder~ (uni=1) & 92.86 & 89.22 & 86.15 & 78.77 \\
\encoder~ (uni=2) & 93.0 & 89.4 & 86.8 & 79.67 \\
\encoder~ (uni=3) & 92.91 & 89.33 & 86.69 & 79.99 \\
BiDi & 93.06 & 89.44 & 85.97 & 80.14 \\
\bottomrule
\end{tabular}
\caption{CoNLL F1 without adapter}
\end{table*}

\begin{table*}[h!]
\small
\centering\begin{tabular}{c c c c c}
\toprule
Model & snips & chunk & ner & srl \\
\midrule
UniDi & 9637 & 78054 & 78041 & 1434190 \\
\encoder~ (uni=1) & 19378.47 & 241717.16 & 241569.97 & 5400964.16 \\
\encoder~ (uni=2) & 30362.21 & 436026.29 & 435879.1 & 10187271.52 \\
\encoder~ (uni=3) & 41345.95 & 630335.42 & 630188.2 & 14973579.72 \\
BiDi & 52329.64 & 824643.68 & 824496.46 & 19759866.11 \\
\bottomrule
\end{tabular}
\caption{Avg GFLOPS per example without adapter}
\end{table*}

\subsection{Difference policy for Adaptive Restarts}



\begin{table*}[h!]
\small
\centering\begin{tabular}{c c c c c c c c}
\toprule
Model & wait=1 & wait=2 & wait=5 & wait=8 & adapter-best & adapter-2nd & oracle \\
\midrule
UniDi & 82.89 & 82.89 & 82.89 & 82.89 & 82.89 & 82.89 & 82.89 \\
\encoder~ (uni=1) & 74.96 & 74.45 & 81.54 & 83.9 & 86.32 & 86.17 & 90.2 \\
\encoder~ (uni=2) & 72.55 & 73.05 & 79.9 & 81.93 & 85.12 & 84.63 & 89.7 \\
\encoder~ (uni=3) & 74.84 & 74.94 & 78.57 & 77.99 & 83.89 & 83.63 & 89.2 \\
BiDi & 75.08 & 69.87 & 68.14 & 66.14 & 82.93 & 82.85 & 87.39 \\
\bottomrule
\end{tabular}
\caption{Streaming EM for SNIPS}
\end{table*}


\begin{table*}[h!]
\small
\centering\begin{tabular}{c c c c c c c c}
\toprule
Model & wait=1 & wait=2 & wait=5 & wait=8 & adapter-best & adapter-2nd & oracle \\
\midrule
UniDi & 72.09 & 72.09 & 72.09 & 72.09 & 72.09 & 72.09 & 72.09 \\
\encoder~ (uni=1) & 78.81 & 79.15 & 77.92 & 75.7 & 82.13 & 81.82 & 84.98 \\
\encoder~ (uni=2) & 79.28 & 79.49 & 78.14 & 75.89 & 82.09 & 81.86 & 85.24 \\
\encoder~ (uni=3) & 79.51 & 79.49 & 77.29 & 74.46 & 81.56 & 81.15 & 85.36 \\
BiDi & 78.67 & 78.33 & 74.07 & 69.58 & 78.19 & 79.11 & 84.57 \\
\bottomrule
\end{tabular}
\caption{Streaming EM for NER}
\end{table*}


\begin{table*}[h!]
\small
\centering\begin{tabular}{c c c c c c c c}
\toprule
Model & wait=1 & wait=2 & wait=5 & wait=8 & adapter-best & adapter-2nd & oracle \\
\midrule
UniDi & 75.76 & 75.76 & 75.76 & 75.76 & 75.76 & 75.76 & 75.76 \\
\encoder~ (uni=1) & 77.55 & 77.52 & 77.18 & 76.63 & 78.43 & 78.23 & 81.9 \\
\encoder~ (uni=2) & 77.72 & 77.72 & 76.72 & 76.05 & 78.17 & 77.89 & 82.41 \\
\encoder~ (uni=3) & 77.67 & 76.78 & 73.92 & 71.89 & 77.67 & 77.48 & 82.16 \\
BiDi & 78.07 & 73.7 & 62.1 & 55.97 & 78.07 & 77.65 & 80.41 \\
\bottomrule
\end{tabular}
\caption{Streaming EM for CHUNK}
\end{table*}



\begin{table*}[h!]
\small
\centering\begin{tabular}{c c c c c c c c}
\toprule
Model & wait=1 & wait=2 & wait=5 & wait=8 & adapter-best & adapter-2nd & oracle \\
\midrule
UniDi & 27.84 & 27.84 & 27.84 & 27.84 & 27.84 & 27.84 & 27.84 \\
\encoder~ (uni=1) & 54.26 & 50.84 & 44.96 & 39.77 & 54.26 & 53.62 & 60.26 \\
\encoder~ (uni=2) & 51.75 & 47.24 & 41.06 & 36.31 & 52.07 & 51.98 & 59.6 \\
\encoder~ (uni=3) & 49.06 & 43.47 & 36.73 & 32.72 & 50.59 & 49.89 & 59.09 \\
BiDi & 43.6 & 35.7 & 32.34 & 32.44 & 54.72 & 49.99 & 61.12 \\
\bottomrule
\end{tabular}
\caption{Streaming EM for SRL}
\end{table*}



\begin{table*}[h!]
\small
\centering\begin{tabular}{c c c c c c c c}
\toprule
Model & wait=1 & wait=2 & wait=5 & wait=8 & adapter-best & adapter-2nd & oracle \\
\midrule
UniDi & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 \\
\encoder~ (uni=1) & 79.07 & 78.21 & 85.0 & 87.3 & 90.22 & 89.98 & 95.21 \\
\encoder~ (uni=2) & 76.31 & 76.3 & 83.35 & 84.91 & 88.53 & 88.05 & 93.9 \\
\encoder~ (uni=3) & 78.2 & 77.93 & 81.55 & 80.84 & 87.18 & 86.86 & 93.17 \\
BiDi & 78.21 & 72.5 & 70.77 & 68.35 & 86.15 & 86.07 & 90.52 \\
\bottomrule
\end{tabular}
\caption{RC for SNIPS}
\end{table*}


\begin{table*}[h!]
\small
\centering\begin{tabular}{c c c c c c c c}
\toprule
Model & wait=1 & wait=2 & wait=5 & wait=8 & adapter-best & adapter-2nd & oracle \\
\midrule
UniDi & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 \\
\encoder~ (uni=1) & 88.23 & 88.54 & 86.33 & 83.29 & 92.24 & 91.52 & 95.2 \\
\encoder~ (uni=2) & 88.15 & 88.3 & 86.05 & 83.01 & 91.54 & 90.85 & 95.18 \\
\encoder~ (uni=3) & 88.25 & 88.15 & 84.95 & 81.17 & 90.71 & 90.01 & 94.79 \\
BiDi & 87.21 & 86.53 & 80.87 & 75.43 & 86.31 & 87.93 & 93.62 \\
\bottomrule
\end{tabular}
\caption{RC for NER}
\end{table*}



\begin{table*}[h!]
\small
\centering\begin{tabular}{c c c c c c c c}
\toprule
Model & wait=1 & wait=2 & wait=5 & wait=8 & adapter-best & adapter-2nd & oracle \\
\midrule
UniDi & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 \\
\encoder~ (uni=1) & 92.82 & 92.24 & 90.79 & 89.5 & 93.9 & 93.32 & 97.24 \\
\encoder~ (uni=2) & 91.87 & 91.2 & 88.92 & 87.22 & 92.26 & 91.58 & 96.47 \\
\encoder~ (uni=3) & 91.55 & 89.87 & 85.05 & 81.84 & 91.55 & 91.15 & 94.96 \\
BiDi & 91.62 & 85.66 & 71.01 & 63.28 & 91.62 & 91.09 & 92.57 \\
\bottomrule
\end{tabular}
\caption{RC for CHUNK}
\end{table*}


\begin{table*}[h!]
\small
\centering\begin{tabular}{c c c c c c c c}
\toprule
Model & wait=1 & wait=2 & wait=5 & wait=8 & adapter-best & adapter-2nd & oracle \\
\midrule
UniDi & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 \\
\encoder~ (uni=1) & 67.89 & 62.88 & 54.51 & 47.83 & 67.89 & 67.1 & 75.42 \\
\encoder~ (uni=2) & 64.62 & 58.1 & 49.25 & 43.12 & 64.54 & 64.53 & 73.66 \\
\encoder~ (uni=3) & 61.46 & 53.53 & 44.05 & 38.65 & 62.45 & 61.81 & 72.3 \\
BiDi & 55.96 & 44.87 & 38.94 & 37.97 & 66.35 & 61.82 & 74.01 \\
\bottomrule
\end{tabular}
\caption{RC for SRL}
\end{table*}


\begin{table*}[h!]
\small
\centering\begin{tabular}{c c c c c c c c}
\toprule
Model & wait=1 & wait=2 & wait=5 & wait=8 & adapter-best & adapter-2nd & oracle \\
\midrule
UniDi & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
\encoder~ (uni=1) & 14.64 & 12.06 & 6.82 & 4.74 & 5.06 & 4.95 & 2.79 \\
\encoder~ (uni=2) & 16.71 & 13.5 & 7.76 & 5.9 & 6.29 & 6.19 & 3.52 \\
\encoder~ (uni=3) & 15.68 & 12.84 & 9.14 & 8.14 & 7.95 & 7.96 & 4.18 \\
BiDi & 15.86 & 17.05 & 15.22 & 14.74 & 9.58 & 9.61 & 5.94 \\
\bottomrule
\end{tabular}
\caption{EO for SNIPS}
\end{table*}


\begin{table*}[h!]
\small
\centering\begin{tabular}{c c c c c c c c}
\toprule
Model & wait=1 & wait=2 & wait=5 & wait=8 & adapter-best & adapter-2nd & oracle \\
\midrule
UniDi & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
\encoder~ (uni=1) & 8.33 & 6.03 & 4.47 & 4.21 & 5.27 & 5.05 & 2.58 \\
\encoder~ (uni=2) & 8.27 & 6.2 & 4.7 & 4.4 & 5.77 & 5.41 & 2.6 \\
\encoder~ (uni=3) & 8.11 & 6.44 & 5.2 & 5.0 & 6.41 & 6.09 & 2.86 \\
BiDi & 8.73 & 7.64 & 7.04 & 6.88 & 6.7 & 8.46 & 3.48 \\
\bottomrule
\end{tabular}
\caption{EO for NER}
\end{table*}


\begin{table*}[h!]
\small
\centering\begin{tabular}{c c c c c c c c}
\toprule
Model & wait=1 & wait=2 & wait=5 & wait=8 & adapter-best & adapter-2nd & oracle \\
\midrule
UniDi & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
\encoder~ (uni=1) & 4.54 & 3.71 & 2.88 & 2.64 & 3.9 & 3.52 & 1.21 \\
\encoder~ (uni=2) & 4.84 & 4.17 & 3.6 & 3.38 & 4.87 & 4.46 & 1.46 \\
\encoder~ (uni=3) & 4.82 & 5.17 & 5.43 & 5.21 & 4.82 & 4.79 & 2.0 \\
BiDi & 4.72 & 8.86 & 12.23 & 12.59 & 4.72 & 5.02 & 3.39 \\
\bottomrule
\end{tabular}
\caption{EO for CHUNK}
\end{table*}

\begin{table*}[h!]
\small
\centering\begin{tabular}{c c c c c c c c}
\toprule
Model & wait=1 & wait=2 & wait=5 & wait=8 & adapter-best & adapter-2nd & oracle \\
\midrule
UniDi & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
\encoder~ (uni=1) & 23.86 & 23.54 & 20.3 & 18.76 & 23.86 & 23.01 & 13.36 \\
\encoder~ (uni=2) & 27.9 & 27.6 & 24.05 & 22.19 & 21.7 & 23.31 & 14.98 \\
\encoder~ (uni=3) & 29.93 & 30.58 & 27.71 & 25.7 & 20.98 & 23.04 & 15.68 \\
BiDi & 33.02 & 35.93 & 33.69 & 31.81 & 18.55 & 24.0 & 15.78 \\
\bottomrule
\end{tabular}
\caption{EO for SRL}
\end{table*}


\begin{table*}[h!]
\small
\centering\begin{tabular}{c c c c c c c c}
\toprule
Model & wait=1 & wait=2 & wait=5 & wait=8 & adapter-best & oracle & adapter-2nd \\
\midrule
UniDi & 9637.44 & 9637.44 & 9637.44 & 9637.44 & 9637.44 & 9637.44 & 9637.44 \\
\encoder~ (uni=1) & 19378.47 & 14479.33 & 11529.97 & 10649.04 & 11633.44 & 9943.32 & 10980.24 \\
\encoder~ (uni=2) & 30362.21 & 19947.54 & 13677.68 & 11804.95 & 15147.97 & 12080.53 & 14220.93 \\
\encoder~ (uni=3) & 41345.95 & 25415.75 & 15825.4 & 12960.85 & 21289.35 & 17060.31 & 20211.03 \\
BiDi & 52329.64 & 30883.9 & 17973.06 & 14116.71 & 35298.71 & 31820.79 & 34908.47 \\
\bottomrule
\end{tabular}
\caption{GFLOPS for SNIPS}
\end{table*}


\begin{table*}[h!]
\small
\centering\begin{tabular}{c c c c c c c c}
\toprule
Model & wait=1 & wait=2 & wait=5 & wait=8 & adapter-best & oracle & adapter-2nd \\
\midrule
UniDi & 78041 & 78041 & 78041 & 78041 & 78041 & 78041 & 78041 \\
\encoder~ (uni=1) & 241569.97 & 156049.74 & 104139.05 & 90967.97 & 241587.24 & 113879.1 & 174277.42 \\
\encoder~ (uni=2) & 435879.1 & 253209.82 & 142329.63 & 114195.72 & 435896.37 & 168436.99 & 289212.77 \\
\encoder~ (uni=3) & 630188.2 & 350369.9 & 180520.2 & 137423.46 & 630205.5 & 242384.54 & 433005.41 \\
BiDi & 824496.46 & 447529.09 & 218709.9 & 160650.34 & 516168.81 & 416556.26 & 824513.76 \\
\bottomrule
\end{tabular}
\caption{GFLOPS for NER}
\end{table*}



\begin{table*}[h!]
\small
\centering\begin{tabular}{c c c c c c c c}
\toprule
Model & wait=1 & wait=2 & wait=5 & wait=8 & adapter-best & oracle & adapter-2nd \\
\midrule
UniDi & 78054 & 78054 & 78054 & 78054 & 78054 & 78054 & 78054 \\
\encoder~ (uni=1) & 241717.16 & 156134.5 & 104185.93 & 91005.21 & 241734.44 & 107961.88 & 178077.13 \\
\encoder~ (uni=2) & 436026.29 & 253294.6 & 142376.5 & 114232.96 & 436043.57 & 174859.72 & 315285.89 \\
\encoder~ (uni=3) & 630335.42 & 350454.68 & 180567.07 & 137460.71 & 630352.72 & 351184.22 & 536950.62 \\
BiDi & 824643.68 & 447613.92 & 218756.78 & 160687.59 & 824660.98 & 720745.14 & 793233.89 \\
\bottomrule
\end{tabular}
\caption{GFLOPS for CHUNK}
\end{table*}

\begin{table*}[h!]
\small
\centering\begin{tabular}{c c c c c c c c}
\toprule
Model & wait=1 & wait=2 & wait=5 & wait=8 & adapter-best & oracle & adapter-2nd \\
\midrule
UniDi & 1434190 & 1434190 & 1434190 & 1434190 & 1434190 & 1434190 & 1434190 \\
\encoder~ (uni=1) & 5400964.16 & 3247558.78 & 1957665.6 & 1630104.3 & 5400985.55 & 4264378.94 & 5024226.32 \\
\encoder~ (uni=2) & 10187271.52 & 5638303.04 & 2913453.74 & 2221496.76 & 8843681.32 & 7824453.98 & 8992399.31 \\
\encoder~ (uni=3) & 14973579.72 & 8029047.1 & 3869241.67 & 2812889.01 & 12271358.54 & 11151910.55 & 12498471.99 \\
BiDi & 19759866.11 & 10419771.02 & 4825008.62 & 3404260.49 & 12504558.49 & 11661925.61 & 13182523.27 \\
\bottomrule
\end{tabular}
\caption{GFLOPS for SRL}
\end{table*}


\begin{table*}[h!]
\small
\centering
\begin{tabular}{| c | c c | c c | c c | c c | c c |}
 \toprule
 Dataset & \multicolumn{2}{|c|}{bi=1} & \multicolumn{2}{|c|}{bi=2} & \multicolumn{2}{|c|}{bi=3} & \multicolumn{2}{|c|}{bi=4} \\
 \midrule
       & Streaming EM & EO & Streaming EM & EO & Streaming EM & EO & Streaming EM & EO \\
 \midrule
 SNIPS & 86.3({\scriptsize 75.0}) & 5.1({\scriptsize 14.6}) & 85.1({\scriptsize 72.5}) & 6.3({\scriptsize 16.7}) & 83.9({\scriptsize 74.8}) & 8.0({\scriptsize 15.7}) & 82.9({\scriptsize 75.1}) & 9.6({\scriptsize 15.9}) \\
 NER & 82.1({\scriptsize 78.8}) & 5.3({\scriptsize 8.3}) & 82.1({\scriptsize 79.3}) & 5.8({\scriptsize 8.3}) & 81.6({\scriptsize 79.5}) & 6.4({\scriptsize 8.1}) & 78.2({\scriptsize 78.7}) & 6.7({\scriptsize 8.7}) \\
 CHUNK & 78.4({\scriptsize 77.5}) & 3.9({\scriptsize 4.5}) & 78.2({\scriptsize 77.7}) & 4.9({\scriptsize 4.8}) & 77.7({\scriptsize 77.7}) & 4.8({\scriptsize 4.8}) & 78.1({\scriptsize 78.1}) & 4.7({\scriptsize 4.7}) \\
 SRL & 54.3({\scriptsize 54.3}) & 23.9({\scriptsize 23.9}) & 52.1({\scriptsize 51.8}) & 21.7({\scriptsize 27.9}) & 50.6({\scriptsize 49.1}) & 21.0({\scriptsize 29.9}) & 54.7({\scriptsize 43.6}) & 18.6({\scriptsize 33.0}) \\

\bottomrule
\end{tabular}
\caption{Streaming Evaluations on Test Set. The number within bracket denotes performance without the ADAPTER. Streaming EM-only = True \label{table:metric_trc-only-True}}
\end{table*}


\begin{table*}[h!]
\small
\centering
\begin{tabular}{| c | c | c | c | c | c |}
 \toprule
 Dataset & bi=0 & bi=1 & bi=2 & bi=3 & bi=4 \\
 \midrule
 SNIPS & 9.6 & 11.6 ({19.4}) & 15.1 ({30.4}) & 21.3 ({41.3}) & 35.3 ({52.3}) \\
 NER & 78.0 & 241.6 ({241.6}) & 435.9 ({435.9}) & 630.2 ({630.2}) & 516.2 ({824.5}) \\
 CHUNK & 78.1 & 241.7 ({241.7}) & 436.0 ({436.0}) & 630.4 ({630.3}) & 824.7 ({824.6}) \\
 SRL & 1434.2 & 5401.0 ({5401.0}) & 8843.7 ({10187.3}) & 12271.4 ({14973.6}) & 12504.6 ({19759.9}) \\

\bottomrule
\end{tabular}
\caption{Streaming GFLOP Evaluations on Test Set with Adapter. The number within bracket denotes performance without the ADAPTER. Streaming EM-only = True \label{table:metric_trc-only-True}}
\end{table*}

\begin{table*}[h!]
\small
\centering
\begin{tabular}{| c | c c | c c | c c | c c |}
 \toprule
 Dataset & \multicolumn{2}{|c|}{bi=1} & \multicolumn{2}{|c|}{bi=2} & \multicolumn{2}{|c|}{bi=3} & \multicolumn{2}{|c|}{bi=4} \\
 \midrule
       & Streaming EM & EO & Streaming EM & EO & Streaming EM & EO & Streaming EM & EO \\
 \midrule
 SNIPS & \textbf{86.1} ({73.7}) & 4.7 ({15.6}) & 85.3 ({71.0}) & 6.0 ({17.6}) & 84.1 ({73.8}) & 8.0 ({16.3}) & 82.5 ({73.3}) & 9.8 ({16.4}) \\
 NER & \textbf{88.0} ({84.2}) & 3.5 ({6.9}) & 87.8 ({84.3}) & 4.0 ({7.0}) & 87.3 ({84.8}) & 4.5 ({6.8}) & 86.0 ({84.2}) & 4.9 ({7.4}) \\
 CHUNK & \textbf{76.7} ({75.5}) & 3.5 ({4.9}) & 76.5 ({75.8}) & 4.5 ({5.2}) & 75.4 ({75.8}) & 5.1 ({5.1}) & 75.6 ({75.8}) & 5.2 ({5.1}) \\
 SRL & 51.9 ({52.6}) & 23.7 ({24.5}) & 50.4 ({50.3}) & 22.4 ({28.7}) & 48.9 ({47.2}) & 21.6 ({30.9}) & \textbf{53.6} ({42.2}) & 19.3 ({34.0}) \\

\bottomrule
\end{tabular}
\caption{Streaming Evaluations on Eval Set. The number within bracket denotes performance without the ADAPTER. Streaming EM-only = False \label{table:eval_metric_trc-only-False}}
\end{table*}

\begin{table*}[h!]
\small
\centering
\begin{tabular}{| c | c | c | c | c | c |}
 \toprule
 Dataset & bi=0 & bi=1 & bi=2 & bi=3 & bi=4 \\
 \midrule
 SNIPS & 9.6 & 10.9 ({19.3}) & 14.6 ({30.1}) & 19.9 ({41.0}) & 34.6 ({51.8}) \\
 NER & 78.0 & 205.3 ({288.4}) & 343.7 ({527.3}) & 517.5 ({766.3}) & 612.7 ({1005.2}) \\
 CHUNK & 78.1 & 210.8 ({288.6}) & 379.6 ({527.5}) & 659.0 ({766.4}) & 972.9 ({1005.3}) \\
 SRL & 1434.2 & 6415.3 ({6910.4}) & 11212.4 ({12994.1}) & 15367.0 ({19077.8}) & 16475.9 ({25161.5}) \\

\bottomrule
\end{tabular}
\caption{Streaming GFLOP Evaluations on Eval Set with Adapter. The number within bracket denotes performance without the ADAPTER. Streaming EM-only = False \label{table:eval_metric_trc-only-False}}
\end{table*}


% \begin{table*}[h!]
% \tiny
% \centering
% \begin{tabular}{| c | c c c | c c c | c c c | c c c | c c c |}
%  \toprule
%  Dataset & \multicolumn{3}{|c|}{bi=0} & \multicolumn{3}{|c|}{bi=1} & \multicolumn{3}{|c|}{bi=2} & \multicolumn{3}{|c|}{bi=3} & \multicolumn{3}{|c|}{bi=4}\\
%  \midrule
%       & Streaming EM & EO & GF &        Streaming EM & EO & GF &     Streaming EM & EO & GF &    Streaming EM & EO & GF &     Streaming EM & EO & GF \\
%  \midrule
%  SNIPS & 82.89 & 0.0 & 9.6 &    86.32 (74.96) & 5.06 (14.64) & 11.6 (19.3) & 85.12 (72.55) & 6.29 (16.71) & 15.1 (30.3) & 83.89 (74.84) & 7.95 (15.68) & & 82.93 (75.08) & 9.58 (15.86) & \\
%  NER   & 72.09 & 0.0 & 78.1 &   82.13 (78.81) & 5.27 (8.33) & & 82.09 (79.28) & 5.77 (8.27) & & 81.56 (79.51) & 6.41 (8.11) & & 78.19 (78.67) & 6.70 (8.73) & \\
%  CHUNK & 75.76 & 0.0 & 78.0 &   78.43 (77.55) & 3.90 (4.54) & & 78.17 (77.72) & 4.87 (4.84) & & 77.67 (77.67) & 4.82 (4.82) & & 78.07 (78.07) & 4.72 (4.72) & \\
%  SRL   & 27.84 & 0.0 & 1434.2 & 54.26 (54.26) & 23.86 (23.86) & & 52.07 (51.75) & 21.7 (27.9) & & 50.59 (40.06) & 20.98 (29.93) & & 54.72 (43.60) & 18.55 (33.02) &  \\
%  \bottomrule
% \end{tabular}
% \caption{Streaming Evaluations on Test Set. The number within bracket denotes performance without the ADAPTER. \ak{How to do hyperparameter selection with two metrics - select two-best based on Streaming EM score, now between these two, I select the one based on lowest FLOP?}}
% \label{offline_test}
% \end{table*}

% \begin{table*}[h!]
% \small
% \centering
% \begin{tabular}{| c | c c | c c | c c | c c | c c |}
%  \toprule
%  Dataset & \multicolumn{2}{|c|}{bi=0} & \multicolumn{2}{|c|}{bi=1} & \multicolumn{2}{|c|}{bi=2} & \multicolumn{2}{|c|}{bi=3} & \multicolumn{2}{|c|}{bi=4}\\
%  \midrule
%       & Streaming EM & EO & Streaming EM & EO & Streaming EM & EO & Streaming EM & EO & Streaming EM & EO \\
%  \midrule
%  SNIPS & 82.89 & 0.0 & 86.32 {\scriptsize (74.96)} & 5.06 (14.64) & 85.12 (72.55) & & 15.1 (30.3) & 83.89 (74.84) & 7.95 (15.68) & \\
% \bottomrule
% \end{tabular}
% \caption{Streaming Evaluations on Test Set. The number within bracket denotes performance without the ADAPTER. \ak{How to do hyperparameter selection with two metrics - select two-best based on Streaming EM score, now between these two, I select the one based on lowest FLOP?}}
% \label{offline_test}
% \end{table*}


\begin{table}[h!]
\small
\centering\begin{tabular}{c c c c c}
    \toprule
    Model        & SNIPS           & CHUNK             & NER            & SRL \\
    \midrule
    UniDi ($bi=0$) & 86.8          & 88.1             & 73.8          & 56.4 \\
    \encoder~ ($bi=1$) & 92.9          & 89.2             & 86.2          & 78.8 \\
    \encoder~ ($bi=2$) & \textbf{93.0} & \textbf{89.4}    & \textbf{86.8} & 79.7 \\
    \encoder~ ($bi=3$) & 92.9          & 89.3             & \textbf{86.7} & \textbf{80.0} \\
    BiDi ($bi=4$)  & \textbf{93.1} & \textbf{89.4}    & 86.0          & \textbf{80.1} \\
    \bottomrule
\end{tabular}
\caption{\label{table:conll_f1_all_debi} Offline F1 of \encoder~ model on test set. We boldface the top-2 performing models for each. The numbers do not reflect state of the art, as these models are smaller and not pretrained\su{no need to show two decimal places. just show XX.X}.}
\end{table}
